From Dragondoom to Dragonstar: Side-channel Attacks and Formally Verified Implementation of WPA3 Dragonfly Handshake

It is universally acknowledged that Wi-Fi communications are important to secure. Thus, the Wi-Fi Alliance published WPA3 in 2018 with a distinctive security feature: it leverages a Password-Authenticated Key Exchange (PAKE) protocol to protect users' passwords from offline dictionary attacks. Unfortunately, soon after its release, several attacks were reported against its implementations, in response to which the protocol was updated in a best-effort manner. In this paper, we show that the proposed mitigations are not enough, especially for a complex protocol to implement even for savvy developers. Indeed, we present **Dragondoom**, a collection of side-channel vulnerabilities of varying strength allowing attackers to recover users' passwords in widely deployed Wi-Fi daemons, such as hostap in its default settings. Our findings target both password conversion methods, namely the default probabilistic hunting-and-pecking and its newly standardized deterministic alternative based on SSWU. We successfully exploit our leakage in practice through microarchitectural mechanisms, and overcome the limited spatial resolution of Flush+Reload. Our attacks outperform previous works in terms of required measurements. Then, driven by the need to end the spiral of patch-and-hack in Dragonfly implementations, we propose **Dragonstar**, an implementation of Dragonfly leveraging a formally verified implementation of the underlying mathematical operations, thereby removing all the related leakage vector. Our implementation relies on HACL*, a formally verified crypto library guaranteeing secret-independence. We design Dragonstar, so that its integration within hostap requires minimal modifications to the existing project. Our experiments show that the performance of HACL*-based hostap is comparable to OpenSSL-based, implying that Dragonstar is both efficient and proved to be leakage-free.

==> resources/bin2bn_code.tex <==
\begin{figure*}
%	\centering
	% Let's make this an lstlisting, not a figure...
	%\makeatletter\def\@captype{lstlisting}\makeatother
	\begin{lrbox}{\verbsavebox}
		\begin{lstlisting}[xrightmargin=.667\linewidth,mathescape=true,
		escapeinside={@}{@},style=codesample,frame=none]
def BN_bin2bn(buf, n, bn):
	# Skip leading zero's
	for ( ; n > 0 && *buf == 0; buf++, n--):	@\label{lst:openssl_impl_bin2bn-opti}@
		continue;

	# Handle special case
	[...]
	
	while (n--):
		# read the bytes in
		[...]
		
	bn_correct_top(ret);
	return ret;
		\end{lstlisting}
	\end{lrbox}
	\subcaptionbox{\textbf{OpenSSL v1.1.1n}\label{lst:openssl_impl_bin2bn}}{\usebox{\verbsavebox}}\hfill%
	\vrule\hfill%
	\begin{lrbox}{\verbsavebox}
		\begin{lstlisting}[xrightmargin=.666\linewidth,mathescape=true,
		escapeinside={@}{@},style=codesample,frame=none]
def mp_read_unsigned_bin(bn, buf, n):
	# Skip leading zero's
	while (c > 0 && b[0] == 0):	@\label{lst:wolfssl_impl_bin2bn-opti}@
		c--; b++;

	# Handle special case
	[...]
	
	mp_zero (bn);
	while (n-- > 0):
		# read the bytes in
		[...]
	mp_clamp (bn);
	return MP_OKAY;
		\end{lstlisting}
	\end{lrbox}
	\subcaptionbox{\textbf{WolfSSL v5.0.0-stable}\label{lst:wolfssl_impl_bin2bn}}{\usebox{\verbsavebox}}\hfill%
	\vrule\hfill%
	\begin{lrbox}{\verbsavebox}
		\begin{lstlisting}[xrightmargin=.666\linewidth,mathescape=true,
		escapeinside={@}{@},style=codesample,frame=none]
def _ecc_be2native(bn, buf, n):
	uint64_t tmp[2 * L_ECC_MAX_DIGITS];
	
	for (i = 0; i < n; i++)
		tmp[n - 1 - i] = l_get_be64(&buf[i]);
	
	memcpy(dest, tmp, n * 8);
		\end{lstlisting}
	\end{lrbox}
	\subcaptionbox{\textbf{ell v0.49}\label{lst:ell_impl_bin2bn}}{\usebox{\verbsavebox}}
	\caption{Implementation of the \code{bin2bn} function in various cryptographic libraries. We extracted only the relevant part, simplified the syntax, and renamed variables to save space.}
	\label{lst:practical_bin2bn}
\end{figure*} 

